Gaussian Process Priors for View-Aware Inference

While frame-independent predictions with deep neural networks have become the prominent solutions to many computer vision tasks, the potential benefits of utilizing correlations between frames have received less attention. Even though probabilistic machine learning provides the ability to encode correlation as prior knowledge for inference, there is a tangible gap between the theory and practice of applying probabilistic methods to modern vision problems. For this, we derive a principled framework to combine information coupling between camera poses (translation and orientation) with deep models. We proposed a novel view kernel that generalizes the standard periodic kernel in $\mathrm{SO}(3)$. We show how this soft-prior knowledge can aid several pose-related vision tasks like novel view synthesis and predict arbitrary points in the latent space of generative models, pointing towards a range of new applications for inter-frame reasoning.

==> fig/chairs/view_cov.tex <==
% This file was created by tikzplotlib v0.9.1.
\begin{tikzpicture}

\begin{axis}[
hide x axis,
hide y axis,
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xmin=-0.5, xmax=59.5,
xtick style={color=black},
y dir=reverse,
y grid style={white!69.0196078431373!black},
ymin=-0.5, ymax=59.5,
ytick style={color=black}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=59.5, ymin=59.5, ymax=-0.5] {view_cov-000.png};
\end{axis}

\end{tikzpicture}


==> fig/chairs/view_cov_test.tex <==
% This file was created by tikzplotlib v0.9.1.
\begin{tikzpicture}

\begin{axis}[
hide x axis,
hide y axis,
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xmin=-0.5, xmax=59.5,
xtick style={color=black},
y dir=reverse,
y grid style={white!69.0196078431373!black},
ymin=-0.5, ymax=59.5,
ytick style={color=black}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=59.5, ymin=59.5, ymax=-0.5] {view_cov_test-000.png};
\end{axis}

\end{tikzpicture}


==> fig/video-interpolation/kernel_face02.tex <==
% This file was created by matplotlib2tikz v0.6.18.
\begin{tikzpicture}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={white!69.01960784313725!black},
xmin=-0.5, xmax=705.5,
y grid style={white!69.01960784313725!black},
ymin=-0.5, ymax=705.5,
width=\figurewidth,
height=\figureheight
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=705.5, ymin=705.5, ymax=-0.5] {fig/video-interpolation/kernel_face02-001.png};
\end{axis}

\end{tikzpicture}

==> fig/video-interpolation/kernel_face03.tex <==
% This file was created by matplotlib2tikz v0.6.18.
\begin{tikzpicture}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={white!69.01960784313725!black},
xmin=-0.5, xmax=350.5,
y grid style={white!69.01960784313725!black},
ymin=-0.5, ymax=350.5,
width=\figurewidth,
height=\figureheight
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=350.5, ymin=350.5, ymax=-0.5] {fig/video-interpolation/kernel_face03-001.png};
\end{axis}

\end{tikzpicture}

==> fig/video-interpolation/kernel_face04.tex <==
% This file was created by matplotlib2tikz v0.6.18.
\begin{tikzpicture}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={white!69.01960784313725!black},
xmin=-0.5, xmax=355.5,
y grid style={white!69.01960784313725!black},
ymin=-0.5, ymax=355.5,
width=\figurewidth,
height=\figureheight
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=355.5, ymin=355.5, ymax=-0.5] {fig/video-interpolation/kernel_face04-000.png};
\end{axis}

\end{tikzpicture}

==> fig/video-interpolation/kernel_face05.tex <==
% This file was created by matplotlib2tikz v0.6.18.
\begin{tikzpicture}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={white!69.01960784313725!black},
xmin=-0.5, xmax=405.5,
y grid style={white!69.01960784313725!black},
ymin=-0.5, ymax=405.5,
width=\figurewidth,
height=\figureheight
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=405.5, ymin=405.5, ymax=-0.5] {fig/video-interpolation/kernel_face05-001.png};
\end{axis}

\end{tikzpicture}
